Towards a Formalism-Based Toolkit for Automotive Applications

The success of a number of projects has been shown to be significantly improved by the use of a formalism. However, there remains an open issue: to what extent can a development process based on a singular formal notation and method succeed. The majority of approaches demonstrate a low level of flexibility by attempting to use a single notation to express all of the different aspects encountered in software development. Often, these approaches leave a number of scalability issues open. We prefer a more eclectic approach. In our experience, the use of a formalism-based toolkit with adequate notations for each development phase is a viable solution. Following this principle, any specific notation is used only where and when it is really suitable and not necessarily over the entire software lifecycle. The approach explored in this article is perhaps slowly emerging in practice - we hope to accelerate its adoption. However, the major challenge is still finding the best way to instantiate it for each specific application scenario. In this work, we describe a development process and method for automotive applications which consists of five phases. The process recognizes the need for having adequate (and tailored) notations (Problem Frames, Requirements State Machine Language, and Event-B) for each development phase as well as direct traceability between the documents produced during each phase. This allows for a stepwise verification/validation of the system under development. The ideas for the formal development method have evolved over two significant case studies carried out in the DEPLOY project.

==> abstract.tex <==
% -*- mode: LaTeX; mode: FlySpell; -*-

\begin{abstract}

%\marginpar{MAJ to confirm affiliation}

%In the automotive industry, software engineering is typically concerned with the development of additional features to existing systems. 
%Frequently, the requirements for --and design of-- a new subsystem will involve only small changes to the existing hardware. 
%The starting point of such a development task is an initial requirements document; 
%the products of the effort are detailed final requirements, a specification document and an implementation. 
%Where these documents are formal, the relationships between them can be reliably established. 
%This paper describes a process for producing the final requirements and the specification document;
%the latter is then the basis for purely formal justification of the final product.
%The process recognises that the requirements must reflect the problem structure while the implementation embodies the solution structure.  
%These ideas have evolved over two significant case studies in Bosch research; 
%they have used Jackson's Problem Frames Approach and Event-B as a formal modelling notation.  
%The process that we outline has the advantage that it will detect problems early. 

%\marginpar{this might be a bit long --- good first para of Introduction --- shorten for Abstract}

%Abstract goes here. Shall be a short version of introduction including problem statemenet and proposed solution.

The success of a number of projects has been shown to be significantly improved by the use 
of a formalism . However, there remains an open issue: 
to what extent can a development process based on a singular
formal notation and method succeed. The majority of approaches 
demonstrate a low level of flexibility by attempting to use a single notation to express all of the different 
aspects encountered in software development. Often, these approaches leave a number of 
scalability issues open. 
We prefer a more eclectic approach.
In our experience, the use of a formalism-based toolkit with adequate notations 
for each development phase is a viable solution. 
Following this principle, any specific notation 
is used only where and when it is really suitable and not necessarily over the entire software lifecycle. 
The approach explored in this article is perhaps slowly emerging in practice ---
we hope to accelerate its adoption.
However, the major challenge is still finding the best way to instantiate it for each 
specific application scenario. In this work, we describe a development process and method for 
automotive applications which consists of five phases. 
The process recognises the need for 
having adequate (and tailored) notations (Problem Frames, Requirements State Machine Language, 
and Event-B) for each development phase as well as direct traceability between the documents
produced during each phase. This allows for a step-wise verification/validation of the system 
under development. The ideas for the formal development method have evolved over two significant 
case studies carried out in the DEPLOY project.

\end{abstract}

